IncShrink: Architecting Efficient Outsourced Databases using Incremental MPC and Differential Privacy

In this paper, we consider secure outsourced growing databases that support view-based query answering. These databases allow untrusted servers to privately maintain a materialized view, such that they can use only the materialized view to process query requests instead of accessing the original data from which the view was derived. To tackle this, we devise a novel view-based secure outsourced growing database framework, Incshrink. The key features of this solution are: (i) Incshrink maintains the view using incremental MPC operators which eliminates the need for a trusted third party upfront, and (ii) to ensure high performance, Incshrink guarantees that the leakage satisfies DP in the presence of updates. To the best of our knowledge, there are no existing systems that have these properties. We demonstrate Incshrink's practical feasibility in terms of efficiency and accuracy with extensive empirical evaluations on real-world datasets and the TPC-ds benchmark. The evaluation results show that Incshrink provides a 3-way trade-off in terms of privacy, accuracy, and efficiency guarantees, and offers at least a 7,800 times performance advantage over standard secure outsourced databases that do not support the view-based query paradigm.

==> 3_problem.tex <==
\section{Problem Formulation}
%\cw{{\bf Assigned to Johes}. I start some initial writing for problem formulation, but feel free to change anyway.}
We formulate our research problem in this section. We first introduce the concept of view-based secure outsourced growing database in Section~\ref{sec:vquery} and then review certain challenges with this design in Section~\ref{sec:challenge}. Lastly we summarize our research objectives in Section~\ref{sec:obj}. 

\eat{A summary of key concepts and notations is provided in Table~\ref{tab:notations}.  
\begin{table}[h]
    \centering
    \begin{tabular}{r|l}
        $u_t$ & logical update at time $t$; can be a single record or null\\
        $\gamma_t$ & real update at $t$, can be a set of records or null\\
        $Sync$ & synchronization strategy; $Sync=\{\gamma_t\}_{t\geq 0}$ \\
        $\mathcal{D}_t$ & logical database at time $t$; $\mathcal{D}_t = \{ u_i \}_{0 \leq i \leq t}$ \\
        $\mathcal{D}$ & the logical instance of a growing database; $\mathcal{D} = \{ u_t \}_{t \geq 0}$\\
        $\mathcal{DS}_t$ & physical data on the server at time $t$ \\
        $\mathcal{DS}$ & the physical data on the server over time\\
        $\mathcal{V}_t$ & materialized view at time $t$ \\
        $\mathcal{V}$ & materialized view over time\\
        $q_t$ & list of queries at time $t$ \\ 
    \end{tabular}
    \caption{Summary of notations.} 
    \label{tab:notations}
\vspace{-4mm}
\end{table}}

\subsection{View-based SOGDB}\label{sec:vquery}
%\cw{revise the logic: (1) view based query asnwering; (2) what is sogdb setting; (3) what is view-based sogdb. (4) evaluation metrics}
The secure outsourced database $(\setup, \update, \query, r\_sync)$~\cite{wang2021dp} is an suite of three secure protocols and a
private record synchronization strategy. This abstracts an encrypted database model among three entities, namely the owner, the server, and the analyst. The owner encrypts and outsources a logical database $\mathcal{D}$ to the server, and continually updates the outsourced database (with new data) via $\update$ protocol. The server stores the outsourced data, $\mathcal{DS}$, on which it process the query (using \query protocol) sent by an authorized analyst. If all potential updates issued by the owner are insertion only, then this is referred as a secure outsourced growing database (SOGDB). In addition, the owner's database update behavior adheres to the private data synchronization policy $r\_sync$, which may not necessarily be the same as the logical updates. For instance, an owner receives a new record every 10 minutes, but may choose to synchronize once her received up to 5 records. 


%The server stores the outsourced data, $\mathcal{DS}$, on which it process the query (using \query protocol) sent by an authorized analyst. Note that, in practice, there could be multiple owners, servers and analysts. 

%For the ease of description, we assume that there may be multiple owners, but they will outsource their logical database to the same server, while the server maintains an independent outsourced database corresponds to each owner. Additionally, we consider there is only one analyst. In the following, we extend this standard model to view-based SOGDB, where the server supports private query answering using materialized views.
 In this work we consider a more efficient approach for processing queries, where queries are answered with a (encrypted) materialized view object $\mathcal{V}$ rather than accessing the underlying outsourced data $\mathcal{DS}$. This allows the server to cache important intermediate results, while avoiding duplicate computations in responding a sequences of pre-specified query workloads~\cite{silberschatz1997database, chowdhury2019crypt}. Typically, materialized views can be transformed solely based on the outsourced data (i.e., filtered tables for outsourced data) or in combination with public information (i.e., a join tables between outsourced data and public relations). We refer the SOGDB with view-based query answering mechanism as the view-based SOGDB. 


%In general, view-based SOGDB is more pragmatic in answering queries on encrypted data, since processing queries on encrypted data usually requires substantial performance overhead, and caching the encrypted intermediate output as materialized views will greatly improve query efficiency~\cite{chowdhury2019crypt}.
%The server rewrites issued queries as linear queries over the

%Typically, the encrypted entries stored in $\mathcal{V}$ are computed over the outsourced data by invoking secure protocols.  Additionally, server-maintained view can also be computed from multiple outsourced databases, i.e. a join table between two outsourced databases belonging to two owners, or combined with public data, i.e. a join table between an outsourced and a public database. Moreover, a view-based SOGDB can be evaluated by the following three dimensions:
\eat{
\boldparagraph{Accuracy}. We use L1 error as the accuracy metric, where L1 error refers to the L1 norm of the difference between the server responded query result and its true result. Formally, assume $q_t$ is the query issued by the analyst at time $t$. Let $\tilde{q}_t(\mathcal{V}_t)$ and $q_t(\mathcal{D}_t)$ denote the result returned by the server in response to $q_t$ and the ground truth result when $q_t$ applies over the logical database $\mathcal{D}_t$, respectively. The aforementioned $\mathcal{V}_t$ denotes the materialized view at time $t$, and $\mathcal{D}_t$ denotes the logical database at $t$, where $\mathcal{D}_t=\{u_i\}_{0\leq i\leq t}$. Then the L1 query error is quantified by $|\tilde{q}_t(\mathcal{V}_t) - {q}_t(\mathcal{D}_t)|$.
    
\boldparagraph{Efficiency}. We use query execution time (QET) as the main efficiency metric, which is the elapse in response of a single query. Note that the QET may be directly related to the size of the materialized view, i.e., the total number of encrypted rows in $\mathcal{V}_t$. Thus, the size of the view can be used as another efficiency indicator.
    
\boldparagraph{Privacy}.~\cite{wang2021dp} pointed out the problem that even with an encrypted database scheme, attackers are still able to infer sensitive information by analyzing the associated leakage when owner updates the outsourced data. In view-based SOGDB system, we consider the owners' data are sensitive. Therefore, each owner would like any other entities' knowledge (other than authorized analysts) about any single update in 
the owner's logical database, $\mathcal{D}$, from observing the update leakage, is bounded by differential privacy. Thus we utilize the privacy parameter $\epsilon$ as the privacy guarantee, and the formal privacy model is later provided in Section~\ref{sec:model}
\eat{
\begin{figure}[h]
\centering
\includegraphics[width=0.96\linewidth]{figures/simpleflow.pdf}
\vspace{-3mm}
\caption{Query response mode.}
\label{fig:cache}
\end{figure}
}
}

\subsection{Main Challenges}\label{sec:challenge}
We briefly review the main challenges of building a view-based SOGDB system.

\boldparagraph{C1. Additional update leakage}. In a standard SOGDB, the update leakage is profiled as the update pattern information~\cite{wang2021dp}, which refers to the transcript of entire data insertion history. Such a pattern may include when each insertion occurs and how many records been inserted at each update. For a view-based SOGDB design, to ensure consistency between the materialized view and the outsourced data, the view needs to be updated alongside the outsourced data. However, the true cardinality of newly transformed view entries (update pattern) also leaks information about the underlying data thus introduces additional update leakage. Although one can alleviate this risk by always packing the newly generated view entries to an exhaustively padded secure array (padded with encrypted dummy tuples to the maximum possible size), or just generate a static view and never update it at all, these na\"ive ways either introduces a large amount of dummy encryptions or causes no utility guarantees. Thus, the first challenge is to balance the utility and efficiency guarantees while mitigating the additional leakage associated with view updating.

\boldparagraph{C2. Potentially unbounded privacy loss}. An alternative way to address C1 is to hide the view update leakage with differential privacy. However, ensuring $\epsilon$-DP with respect to the view instance does not imply $\epsilon$-DP to the logical data where the view is derived. This is because an individual data point in the logical database may contribute to generating multiple view entries. As a result, the framework either incurs an unbounded privacy loss or has to stop updating the materialized view after enough updates. This leads to the second challenge, which is to support unlimited times of view updates while ensure fixed privacy loss.

%Providing privacy guarantee with respect to a view instance does not implies the same privacy guarantee for the original relations where the view is  derived. This is because an individual data point in the underlying data may contribute to generating multiple view entries. %Thus even if the membership information of one view entry is preserved, an attacker could also infer the membership information of the source data by o

\boldparagraph{C3. Maintaining encrypted materialisation over untrustworthy entity}
%\cw{We may want a shorter section for naive approaches}
%The key aspect of extending the standard SOGDB to a view-based SOGDB is to design security protocols that maintain encrypted materialized views. We start discussing some na\"ive design options.

\eat{
\boldparagraph{Simultaneously updated view (SUV)} \cw{Perhaps we can skip this method as it's non-private and we never compared it in out experiments}. There are several na\"ive design concepts to extend the standard SOGDB to a view-based SOGDB, the most intuitive method is to have the server maintain a materialized view with growing entries that is updated simultaneously with the user's outsourced data. More specifically, the owners update their outsourced data independently with the new data. On the server side, whenever the outsourced database is updated, the server invokes a secure protocol (i.e. MPC, TEE or homomorphic encryption based secure computing protocol) to compute potential new entries for the materialized view. The protocol outputs the encrypted new entries, which are then added to the materialized view by the server. This approach ensures that the view is always consistent with the outsourced data. However, SUV is a non-private method as it reveals the exact number of newly added entries to the view. 

\boldparagraph{One-time materialization (OTM)}. To remedy the privacy issue of SUV, the server can generate a static view at the initial stage and never update it. Since no updates occur on the materialized view, no additional leakage are thus revealed. However, the gap between the outsourced data and the view will keep increasing and therefore produce inaccurate query results.

\boldparagraph{Exhaustive padding (EP)}. Another private approach is to have the server update the view simultaneously with the user's outsourced data. But each time the materialized view is updated, the server pads the newly added view entries with additional dummy entries to bring it to the maximum possible size. This guarantees the view is always consistent with the outsourced data and also ensures the number of true entries inserted to the view is hidden by exhaustive padding. Obviously, this approach may introduce a large amount of bogus data, which may result in a significant increase in performance overhead in response to queries}

\subsection{Research Objectives}\label{sec:obj}
The na\"ive approaches show that there is a trade-off between the privacy, efficiency and the accuracy guarantee. All na\"ive approaches achieve two of these dimensions, but not the third, which means that when such a design is adopted, users must completely sacrifice one of these dimensions in exchange of their desired goal. For example, if users prefer to have high privacy guarantees, then they must completely sacrifice accuracy (OTM) or efficiency (EP). Such an inflexible design is not practical, and in general users may be willing to make some sacrifices in one dimension in exchange for enhancements in other dimensions, but they may not want to give up one dimension of guarantee entirely. Navigating the design space of materialized view update protocols requires balancing a 3-way trade-off between privacy, accuracy, and performance. Furthermore, the untrustworthy server will be the primary subject that continuously update the materialized view, therefore the protocol used to maintain the materialized view must ensure no additional leakages that allow the server to infer sensitive information about the owner's data are are exposed. Inspired by these, we now formulate our research objectives as follows:
\begin{itemize}
    \item Build a generic framework that extends a standard SOGDB system to a view-based SOGDB.
    \item Design secure protocols to continually update the materialized view such that (i) it can be evaluated by potentially untrusted entities and (ii) it balances the trade-off between privacy, accuracy and efficiency.
    \item Ensures bounded privacy loss and provides unlimited updates to the materialized view..
\end{itemize}



%record synchronization policy developed by DP-Sync~\cite{wang2021dp}, we design corresponding strategies for privately updating the materialized join structure. 


%However, unlike the setup in DP-Sync where the sync algorithms are executed by the \user herself, the private strategies for updating the materialized join structure have to be executed on the untrusted server. Naively deploying DP-Sync's synchronization policies to update the materialized join structure can lead to additional leakage, i.e., the true count of new joins inserted at each time. Therefore, to ensure that the update strategies can be carried out over untrustworthy platforms without violating our established privacy model, we utilize cryptographic primitives such as MPC, secret sharing, and secure outsourcing caches to assist us in designing the update algorithm. 




==> fig.tex <==
\begin{figure}[h]
\captionsetup[sub]{font=small,labelfont={bf,sf}}
    \begin{subfigure}[b]{0.48\linewidth}
    \centering    \includegraphics[width=1\linewidth]{figures/dp_cmp/tpcds_0.1_acc.pdf}
        \caption{TPC-ds L1 error with $\epsilon=0.1$}
        \label{fig:acc-q1-0.1}\end{subfigure}%%
    \begin{subfigure}[b]{0.48\linewidth}
    \centering    \includegraphics[width=1\linewidth]{figures/dp_cmp/cpdb_0.1_acc.pdf}  
        \caption{TPC-ds QET with $\epsilon=0.1$}
        \label{fig:perf-q1-0.1}
    \end{subfigure}
    \newline
    \begin{subfigure}[b]{0.48\linewidth}
    \centering    \includegraphics[width=1\linewidth]{figures/dp_cmp/tpcds_1_acc.pdf}
        \caption{CPDB L1 error with $\epsilon=0.1$}
        \label{fig:acc-q2-0.1}\end{subfigure}%%
      \begin{subfigure}[b]{0.48\linewidth}
    \centering    \includegraphics[width=1\linewidth]{figures/dp_cmp/cpdb_1_acc.pdf}  
        \caption{CPDB QET with $\epsilon=0.1$}
        \label{fig:perf-q2-0.1}
    \end{subfigure}
    \newline
    \begin{subfigure}[b]{0.48\linewidth}
    \centering    \includegraphics[width=1\linewidth]{figures/dp_cmp/tpcds_10_acc.pdf}
        \caption{TPCds L1 error with $\epsilon=10$}
        \label{fig:acc-q2-0.1}\end{subfigure}%%
      \begin{subfigure}[b]{0.48\linewidth}
    \centering    \includegraphics[width=1\linewidth]{figures/dp_cmp/cpdb_10_acc.pdf}  
        \caption{CPDB L1 error with $\epsilon=10$}
        \label{fig:perf-q2-0.1}
    \end{subfigure}
    \newline
    \vspace{-2mm}
   \caption{DP-Timer vs. DP-ANT} \vspace{-4mm}
   \label{fig:q-acc}
\end{figure}

==> removed_proofs.tex <==
\eat{
We start with the definition load overestimation.

\begin{definition}[Load Overestimation] Given two vectors ${\bf u} = \{u_1, u_2, ...,u_n\}$, and ${\bf v} = \{v_1, v_2,...,v_n\}$, we write ${\bf u} \leq {\bf v}$ if for any $\forall 1\leq i \leq n$, it has $u_i \leq v_i$. Then given $X \in \mathbb{R}^{k}$, where $X = \{x_1, x_2, ...,x_k\}$. A random function $\tilde{\textbf{Ld}}(X)$ is said to be a load overestimation of $X$ if the probability $\textup{Pr}[X \leq \tilde{\textbf{Ld}}(X)]$ is overwhelming. 
\end{definition}

Then let $C = \{c_1, c_2, ..., c_k\}$ denotes the collections of join table size at each (join) updates, and $c_i \in C$ denote the true join table size at $i^{th}$ (join) updates. Then Algorithm~\ref{algo:cbuffer} distorts $C$.


\begin{algorithm}[]
\caption{Differentially Private Load Overestimation}
\begin{algorithmic}[1]
\Statex
\textbf{Input}: \\
True join table size $C = \{c_1, c_2, ..., c_k\}$\\
Privacy budget $\epsilon$ \\
Threshold $\theta$\\
Safe buffer $z_1, z_2$\\
%\Statex
\State $\epsilon_1 \gets \frac{1}{2}\epsilon, \epsilon_2 \gets \frac{1}{2}\epsilon$
\State {\bf output} $\tilde{c}_1 \gets c_1 + \lap(\frac{1}{\epsilon_1}) + z_1$
\State $o \gets \tilde{c_1}$
\State $o^{*} \gets \max(o - z_2, 0)$, $\tilde{\theta} \gets \theta + \lap(\frac{2}{\epsilon_2})$
\For{$t \leftarrow 2,...$} %\kartik{consistency with $\gets$, $=$}
\State $v_t \leftarrow \lap(\frac{4}{\epsilon_2})$
\State $q_t\gets |c_t - o*| $
\If{$q_t + v_t \geq \tilde{\theta}$}
\State {\bf output} $\tilde{c}_t \gets c_t + \lap(\frac{1}{\epsilon_1}) + z_1$
\State $o \gets \tilde{c}_t$, $o^{*} \gets \max(o - z_2, 0)$, $\tilde{\theta} \gets \theta + \lap(\frac{2}{\epsilon_2})$
\Else 
\State {\bf output} $\tilde{c}_t \gets o$
\EndIf
\EndFor
\end{algorithmic}
\label{algo:cbuffer}
\end{algorithm}

\begin{theorem}[Sketch] Let the safe buffer (Algorithm~\ref{algo:cbuffer}) $z_1 \gets \frac{2\log(1/\beta)}{\epsilon_1}$, and let $z_2 \gets \theta + \frac{4\log t + 4\log(1/\beta)}{\epsilon_2}$. Then for any time $t$, with probability at least $1-\beta$ it satisfies $\textup{Pr}[c_t \leq \tilde{c}_t]$.
\end{theorem}
\begin{proof}
First, assume for all $t'$ such that $\tilde{c_{t'}}$ is generated by adding Laplace noises (Alg2:15). Then we know that 

\begin{equation}
\begin{split}
& \textup{Pr}\left[\lap(\frac{1}{\epsilon_1}) \leq -\frac{2\log(1/\beta)}{\epsilon_1} \right] \leq \beta \\
\rightarrow & \textup{Pr}\left[\lap(\frac{1}{\epsilon_1}) + z_1 \leq z_1 -\frac{2\log(1/\beta)}{\epsilon_1} \right] \leq \beta\\
\rightarrow & \textup{Pr}\left[\tilde{c_{t'}} - c_{t'} \leq 0 \right] \leq \beta
\end{split}
\end{equation}.

Then we assume all $t^*$ such that $\tilde{c}_{t^*}$ is approximated by previous release. We know that for any $q_{t^*}$, it satisfies that 

\begin{equation}
\begin{split}
& \textup{Pr}\left[q_{t^*} - \theta \geq \frac{4\log t + 4\log(1/\beta)}{\epsilon_2} \right] \leq \beta \\
\rightarrow & \textup{Pr}\left[q_{t^*} \geq \theta + \frac{4\log t + 4\log(1/\beta)}{\epsilon_2} \right] \leq \beta\\
\rightarrow & \textup{Pr}\left[c_{t^*} - o + z_2 \geq \theta + \frac{4\log t + 4\log(1/\beta)}{\epsilon_2} \right] \leq \frac{\beta}{2}\\
\rightarrow & \textup{Pr}\left[c_{t^*} - o \geq 0 \right] \leq \frac{\beta}{2} \rightarrow  \textup{Pr}\left[\tilde{c_{t^*}} - c_{t^*} \leq 0 \right] \leq \frac{\beta}{2}\\
\end{split}
\end{equation}.

Thus the claim holds.
\end{proof}

\begin{theorem}
Let $\mathcal{M}$ be a mechanism that takes a growing database $\mathcal{D}$ as the input, and output a transcript ${\bf o} = \{o_1, o_2, o_3,...\}$. Suppose $\mathcal{M}$ can be decomposed to sub-mechanisms with $\mathcal{M} = \{\mathcal{M}_t\}_{t\geq 0}$, where $\mathcal{M}_t$ takes as input of a sub stream $\{u_{i-w+1}, u_{i-w+2}, ...,u_i\}\subseteq U_t$. If each sub-mechanism $\mathcal{M}_i$ satisfies $\epsilon_i$-DP, then $\mathcal{M}$ satisfies $\epsilon$-DP if: $\forall 0\leq i \leq t, \sum_{i-w+1}^{i} \epsilon_i \leq \epsilon$
\end{theorem}
\begin{proof}
Since all the mechanisms use independent randomness, the following holds for stream prefix $U_t$ and any mechanism output ${\bf o} = (o_1, o_2, ...,o_t)$. 
$$\textup{Pr}[\mathcal{M}(U_t) = (o_1, o_2, ...,o_t)] = \Pi_{i=1}^{t}\textup{Pr}[\mathcal{M}_i(U_t^{i}) = o_i]$$,
where $U_t^i$ denotes the sub stream $\{u_{t-w+1}, ..., u_i\}$ Assume $U_t$ and $U'_t$ are neighboring stream prefix that satisfies $\forall i\neq j, u_i=u'_i$, and $u_j\neq u'_j$. Then we computing the following ratio:
\begin{equation}
    \begin{split}
        \frac{\textup{Pr}[\mathcal{M}(U_t) = {\bf o}]}{\textup{Pr}[\mathcal{M}(U'_t) = {\bf o}]} & = \Pi_{i=0}^{t}\frac{\textup{Pr}[\mathcal{M}_i(U^i_t) = o_i]}{\textup{Pr}[\mathcal{M}_i(U'^i_t) = o_i]}\\
        & = \Pi_{i=0}^{j-1}\frac{\textup{Pr}[\mathcal{M}_i(U^i_t) = o_i]}{\textup{Pr}[\mathcal{M}_i(U'^i_t) = o_i]} \times \Pi_{i= j + w}^{t}\frac{\textup{Pr}[\mathcal{M}_i(U^i_t) = o_i]}{\textup{Pr}[\mathcal{M}_i(U'^i_t) = o_i]}\\
        & \times \Pi_{i=j}^{j + w -1}\frac{\textup{Pr}[\mathcal{M}_i(U^i_t) = o_i]}{\textup{Pr}[\mathcal{M}_i(U'^i_t) = o_i]}\\
        & \leq  \sum_{i=j}^{j+w-1} \epsilon_{i} \leq \epsilon
    \end{split}
\end{equation}
\end{proof}
}

==> revision_letter.tex <==

%%
%% The "title" command has an optional parameter,
%% allowing the author to define a "short title" to be used in page headers.

\begin{center}
\textbf{Revision Letter: Paper \#400 \\ IncShrink: Architecting Efficient Outsourced Databases using Incremental MPC and Differential Privacy}
\end{center}


We would like to thank the reviewers for their detailed and thoughtful comments, which have helped us to significantly revise our paper in terms of completeness and readability. We have \textcolor{blue}{highlighted all new text in the main paper} for ease of reference.  The following section outlines the main changes to the paper. %‚Äì (a) improved discussion on how to extend \system for the malicious adversary model, (b) experiments on larger dataset and (c) text revisions for improved paper readability
%while in Section 2, we address each reviewer's comment individually.
\subsection*{Summary of Changes}
%We denote the $i^{th}$ comment mentioned under ``opportunities for improvment" in review 1 as R1O$i$. 
All the citations in the revision letter refer to corresponding citations in the main paper.

\vspace{1.5mm}
\stitle{Meta Review 1: Clarify the novelty of this work compared to~\cite{ bater2017smcql, bater2018shrinkwrap, wang2021dp}}. We have provided an expanded discussion in Section~\ref{sec:related} that highlights the differences between our work and important related efforts~\cite{bater2017smcql, bater2018shrinkwrap, wang2021dp}. We have also improved the discussions in Section~\ref{sec:pre} and ~\ref{sec:dp-st} to better illustrate the key differences between our design and the closely related works~\cite{bater2018shrinkwrap, wang2021dp}, as well as our technical novelties. Throughout the discussions, we: (i) Explain why the existing efforts~\cite{bater2018shrinkwrap, wang2021dp} do not meet our target design objectives; (ii) Elaborate on what new challenges need to be addressed in light of our privacy promise and design goals; and (iii) Highlight what new technologies and designs we have adopted to address the aforementioned potential challenges.

%We emphasize that~\cite{ bater2017smcql} neither considers handling dynamic data nor attempts to use DP to hide any side channel leakage, and thus is quite different from our work. Also, in the original text (Section~\ref{sec:related}), we have listed~\cite{bater2017smcql} together with some similar works and explained that the main leakage addressed by \system is different from the listed works. Therefore, for space concerns, we did not provide a separate comparison between~\cite{bater2017smcql} and our work. \ashwin{This is the top meta reviewer concern. So we can not ignore it due to space concerns. We need to add a line or two comparing to [6].}
%In the beginning of sections~\ref{sec:pre} and~\ref{sec:dp-st}, we have discussed the potential challenges of designing $\trans$ and $\sync$ protocols, explained why we cannot simply leverage designs from previous works, and summarized our additional designs or implementations. We believe these discussions are necessary to articulate our novelty as well, thus we left these paragraphs unchanged. \ashwin{Does this address [6, 7] or [81]?}


\vspace{1.5mm}
\stitle{Meta Review 2: Expand the discussion on how many servers you can support}. We have provided an independent paragraph in Section~\ref{sec:ext} (extend to multiple servers) to discuss how to extend our \system design to work with multiple servers. We emphasize that our current design can be adapted to a $N\geq 2$ servers setup as long as at least one of the $N$ servers is not colluding with any others. Moreover, in this extended discussion, we have summarized the key modifications that would expand our current design to a multiple server setup. 

\vspace{1.5mm}
\stitle{Meta Review 3: Clarify the privacy guarantee of \system (especially, discuss the cases when each user contributes an unknown amount of records or the updates are correlated)}. We have provided an extended discussion on our privacy guarantees in Section~\ref{sec:privacy}. The main discussions w.r.t. this meta review comments are listed as follows: (i) we clarified that we focus primarily on event-level privacy and (ii) we discussed the fact that event-DP with parameter $\epsilon$ can simultaneously provide DP guarantees for properties across multiple updates (or the records are correlated) at the user level, but may have a different privacy parameter $\epsilon'$. Typically $\epsilon'$ should be larger than $\epsilon$ but no more than $\ell\times\epsilon$, where $\ell$ is the maximum number of records owned by a single user. Note that even without knowing the potential correlations or the number of records owned by each user, one can still derive an upper bound on $\epsilon'$ by setting $\epsilon$ to a pessimistic large value. Moreover, recent works~\cite{cao2017quantifying, song2017pufferfish} indicate that, with some knowledge of correlations, one can derive tighter bounds for $\epsilon'$. 
%\ashwin{Say that with knowledge of correlations one can derive tighter bounds using https://arxiv.org/abs/1603.03977, https://arxiv.org/abs/1610.07543. }

\vspace{1.5mm}
\stitle{Meta Review 4: Discuss the impact of different Truncation bound $\omega$ and provide additional experiments}. We have provided additional discussions and experimental results (in Section~\ref{sec:exp-omega}) investigating the impact of different truncation bounds $\omega$ on the \system framework. In this additional section, evaluate \system over different truncation bounds ranging from $2$ to $32$, and studied how $\omega$ would affect \system in terms of query accuracy (L1-error), query efficiency (QET), and the view update protocol execution timings. The corresponding experiment result is reported in Figure~\ref{fig:trunc}.
%Furthermore, we also explained the rational behind such effects raised by different truncation bounds $\omega$. %\ashwin{I do not understand the last sentence. Did you mean we ``interpret the impact of $\omega$ on accuracy/efficiency metrics"?}


%\cw{complete this after exps}

\vspace{1.5mm}
\stitle{Meta Review 5: Discuss when and how \system returns inaccurate results}. We have provided additional discussions on how and when \system produces inaccurate query results in Section~\ref{sec:dp-timer-detail}. In general, the query errors are caused by (i) the true data discarded by $\trans$ protocol due to the truncation constraint and (ii) the total amount of unsynchronized view tuples (cached data). We also studied experimentally how truncation bound would affect query errors in Section~\ref{sec:exp-omega}. Nevertheless, one could still choose a relatively large truncation bound $\omega$ to ensure that no valid view tuple is discarded by $\trans$. In such cases, the query errors are mainly caused by the number of unsynchronized view tuples. These cached data should be part of the materialized view, but since they are not yet synchronized, will not be used for query processing, and 
thus resulting in query errors. It is not hard to see that less cached data that satisfies the requesting query would imply better query accuracy. Additionally, in the original text, we have provided theoretical upper bounds (Theorem~\ref{lg:timer} and ~\ref{one:ant}) on the amount of cached data, which can be used to theoretically learn the upper bounds for query errors as well.
%\ashwin{SOLVED: -- The errors from (i) and (ii) seem different to me. Can't we, in principle, return the tuples in the cache (ii) to the user to make for that error? Note that R4O2 actually suggests scanning the cache.  But looks like errors in (i) can not be recovered from?} 
%\ashwin{What does having a large truncation threshold entail? Does it slow down run time performance? }

%\ashwin{Did we have to remove anything to make space for all these additions?}

\vspace{2mm}
\stitle{Other changes}. Some other changes in addition to the meta review comments are summarized as follows:
\begin{itemize}
    \item We fixed typos and improved some descriptions to make them more rigorous.
\end{itemize}

\subsection*{Individual Reviewer Comments}
We address the comments of individual reviewers in this section, and please note that we may not include comments that are beyond the scope of the meta-review comments.\\

\boldparagraph{Reviewer \#4}\\
%\noindent\textit{R4O1. For completeness, it would be relevant to include an insecure plaintext database for comparison (e.g. PostgreSQL).I understand why you only included the solutions that work in your security model, but one should still be able to see the added overhead of protecting the update pattern as opposed to not protecting.}\\
%Since the this review comment does not appear in the Meta-review comments.  Therefore, we did not provide relevant modifications with respect to this comment in the main body of the revised paper.\ashwin{This is brutally honest, but the reviewer will not appreciate it. Maybe not mention this comment in the letter.}\\
\noindent\textit{R4O2. I would recommend expanding the discussion on when and how your solution returns inaccurate response. Can (and should) the analyst at least know that the given query results in inaccurate response? Is it possible to scan the cache upon query so these values are not lost?.}\\

We have provided extended discussions in Section~\ref{sec:dp-timer-detail} on how and when \system produces inaccurate query results. The query errors of \system are caused by two factors, namely, the total records discarded by the $\trans$ protocol due to truncation constraints and the total amount of unsynchronized data in the cache. We also experimentally investigated how truncation bounds would affect query errors in Section~\ref{sec:exp-omega}, and based on the results, we observed a significant increase in query errors returned by \system when the truncation bound is relatively small. Nevertheless, one could still pick a relatively large truncation bound, i.e. a pessimistic large estimation of $\omega$, to ensure that no data is discarded by $\trans$.

When a relatively large $\omega$ is selected (assuming no real tuples are discarded by $\trans$), then query errors are mainly caused by unsynchronized view tuples. This is because by default, unsynchronized view tuples (cached data) are not used for secure query processing, even if they are stored on the servers. Typically, less unsynchronized data that satisfy the requesting query means better accuracy and vice versa. Furthermore, we stress that scanning the cache upon answering the query (or returning the entire cache to the client) is a valid strategy and will not break the security promise. This also eliminates errors caused by unsynchronized data, but increases the runtime overhead ( either in terms of server computation costs or communication costs) because the entire cache is exhaustively padded with dummy data. Additionally, in our evaluations (Section~\ref{sec:exp}), we have found that even without scanning the cache (or returning the cache back to the client) the relative query errors under all test groups are small (i.e. bounded by 0.043).\\ 
%\ashwin{SOLVED:We should break this response into two paragraphs -- one about truncation threshold and another about unsynchronized updates. I think we should acknowledge that returning the cache (or scanning it to answer the query) is a valid strategy and will not breack the security promise. This will, however, increase the runtime overhead (either on the client or on the server). You can end by saying that even without scanning the cache we find that the errors are small. We should add this discussion about returning the cache or processing the query on the cache in the main paper.}\\


\noindent\textit{R4O3. I recommend you expand the discussion on how many servers you can support. So far it seems 2 servers is the only configuration. Does it make sense to support more? Is it possible? Will it add any overhead?}\\

We have provided an additional subsection in Section~\ref{sec:ext} that discusses how to adapt our current framework design to work with $N$ servers such that $N\geq2$ under the assumption that the attackers can corrupt all but one server. \\

\eat{
\boldparagraph{Reviewer \#5}\\
\noindent\textit{R5O1. This paper focuses on the fairly limited use case of fixed queries over a monotonically-growing database. That said, a number of interesting use cases exist within these assumptions. Further, Section 8 explore the possibility of extensions to this basic model.}\nt{How to respond to this comment? It seems this comment does not appear in the meta-review comment.}\ashwin{I think we should add a line or two in the motivation of the paper citing work on systems that answer fixed \textit{continuous queries} over a growing (\textit{or streaming}) databases. There are several such systems in the database literature.}\\
}

\boldparagraph{Reviewer \#6}\\
\noindent\textit{R6O1. The technical contribution of this work may be incremental to~\cite{wang2021dp} and~\cite{bater2018shrinkwrap}. Although the key idea KI-1 of using materialized view to query dynmical database securely may be interesting, the other two key ideas are straightforward. The MPC protocol and DP-protected updates proposed in this work are built on existing work~\cite{bater2018shrinkwrap} and~\cite{wang2021dp}. For example, the shrink protocol with Timer-based (sDPTimer) algorithm and Above noisy threshold (sDPANT) algorithm (and the related theorems) is just a straightforward extension from~\cite{wang2021dp}'s Timer-based synchronization and Above noisy threshold (DP-ANT) algorithms.The authors may want to clarify the novelty regarding the above concerns.}\\

We have provided an expanded discussion in Section~\ref{sec:related} that highlights the differences between our work and closely related efforts~\cite{bater2017smcql, bater2018shrinkwrap, wang2021dp}. We have also improved the discussions in Section~\ref{sec:pre} and ~\ref{sec:dp-st} to better illustrate the key differences between our design and the closely related works~\cite{bater2018shrinkwrap, wang2021dp}, as well as our technical novelties. In general, the main security promise of~\cite{bater2017smcql} is to conceal the data values, so it does not consider addressing important side-channel volume leakage, such as the output size of secure operators. Though~\cite{bater2018shrinkwrap} hides the output volume of secure operators and implements a similar resizing method, their resizing is a one-shot operation and is composed as a one-time MPC. Thus the main focus of~\cite{bater2018shrinkwrap} is to handle static data. However, in \system, we split the view update function into two separate but collaborative incremental MPC steps, so that servers can continuously transform new data to view entries while privately synchronizing views with reduced sizes at the same time. In addition, this separated design provides flexibility in choosing different view update strategies. For example, one may want to update the materialized view at a fixed interval or update it when there are enough new view entries. Each time one needs to switch between these two strategies, she only needs to recompile the $\sync$ protocol without making any changes to the $\trans$ protocol. \cite{wang2021dp} only considers a na\"ive query mode, while \system employs a view-based query mode. Additionally,~\cite{wang2021dp} assumes sync strategies are enforced by trusted entities, however, in our setup, $\sync$ is evaluated by two untrusted servers. Na\"ively adopting strategies in~\cite{wang2021dp} could lead to additional leakage to untrusted servers, such as internal randomness. To address these, we made non-trivial re-designs such as adopting joint noise adding mechanism so that no one can control or guess the randomness that derives the DP noise. We also carefully designed the $\trans$ protocol to privately maintain a secure cardinality counter, which is passed to $\sync$ as the auxiliary input to help with the generation of noisy cardinalities. \\


%In addition to that, in the original text, at the begining of sections~\ref{sec:pre} and~\ref{sec:dp-st} \ashwin{I see no new text in 5.1. Maybe the reviewer did not read this? Is there a way we can modify it a bit so we can highlight it and bring it to the attention of the reviewer?}, we have discussed the main challenges in designing $\trans$ and $\sync$ protocols and explained why the existing solutions do not meet the requirements.

%$We summarized the key modifications, re-designs and additional implementations in our \system framework which are apparently not trivial extensions from~\cite{bater2018shrinkwrap, wang2021dp}.\ashwin{I think you say the same thing in the three sentences here. Instead you should state a summary of why you think we are novel and then say this discuss is included in Section 5.1 and 5.2. }\\

\noindent\textit{R6O2. This work considers logical queries (updates), which is not a typical relational database scenario. The authors may want to justify why the logical database could be (or how it can be easily extended to) a general setting.(i) This work assumes only two untrusted servers, which may not apply to multiple servers. (ii) The neighboring growing databases are defined in an event-level DP manner, which may not be a reasonable way to guarantee the privacy of update patterns, which may occur in multiple updates. (iii) The authors may overstate that the proposed protocols can be adapted to underlying secure outsourced database schemes such as MPC, HE, TEE, etc. If I'm not mistaken, the proposed protocols only work for server-aided MPC. (iv) The authors assume that data owners submit a fixed amount of data at fixed intervals.}\\

\begin{itemize}
    \item (i) We have provided an additional subsection in Section~\ref{sec:ext} that discusses how to adapt our current framework design to work with $N$ servers such that $N>2$ under the assumption that the attackers can corrupt all but one server.
    \item (ii) We have provided an extended discussion on our privacy guarantees and justified our choice of privacy notation in Section~\ref{sec:privacy}. We stress that in this paper we focus on event-level privacy with parameter $\epsilon$. However, due to the group-privacy property of DP, one can achieve privacy for properties across multiple updates at the user level as long as the property depends on a finite number of updates. Moreover, there are settings where each update is indeed a new individual’s record. For example, in the election use case, each voter is restricted to vote only once. Thus, each voting record can only correspond to one individual. Event-level DP suffices in this setting.
    \item (iii) As per~\cite{kamara2011outsourcing}, server-aided 2pc design can be directly used for general MPC applications where an arbitrary number of parties provide their confidential inputs. Thus it’s not hard to adapt our framework to databases under general MPC settings. Implementing our operations in TEE or HE would require working out additional details which we have not included due to space constraints. Nevertheless, all we are claiming is that it is feasible to extend the high-level designs (i.e. the “Trans-Shrink” paradigm, the trans\_truncate operator, the view update methods, etc.) to these settings. 
    \item (iv) In the original text (Section~\ref{sec:ext}), we have discussed that owners are not subject to specific data upload behaviors, such as submitting a fixed amount of data at a fixed interval. The owners may choose other uploading strategies such as adopting DP-Sync~\cite{wang2021dp}.\\
\end{itemize}

\noindent\textit{R6O3. A key parameter truncation bound $\omega$ is not thoroughly studied. Questions like how to determine $\omega$ for arbitrary queries and how $\omega$ may affect the 3-way tradeoff need to be theoretically and experimentally answered.}\\

We have conducted additional experiments and provided experimental results on investigating the effects of different truncation bounds $\omega$ in Section~\ref{sec:exp-omega}. Note that when $\omega$ is too small, then a large number of true view tuples will be dropped out by $\trans$ protocol due to the truncation constraint. Thus by default, in our setting  we set $w$ to a pessimistic large value, such as $w$ is equal to the maximum possible contribution of a single input data. Please note that recent work~\cite{kotsogiannis2019privatesql} studied how to dynamically learn truncation bounds for arbitrary queries, we consider this as an interesting future work to support their technique in \system.\\


\noindent\textit{R6O4. This work would be more interesting if the authors further studied the "extensions" discussed in sec8.}\\

We have provided more discussions as suggested by the meta-review comments, such as how to extend our setting to work with more than two servers in Section~\ref{sec:ext}. 



\newpage


==> security.tex <==
\section{Security Model}
\subsection{DP Mechanism with Sliding Window}
\begin{table}[h]
    \centering
    \begin{tabular}{r|l}
        $\mathcal{D}_x$ & the logical database for party $A$ or $B$, where $x\in(A,B)$.   \\
        $\mathcal{D}_x(t)$& logical database at time $t$ for corresponding party.\\
        $T$ & collection of time stamps when recomputes joint tables.
    \end{tabular}
    \caption{Summary of notations.} 
    \label{tab:notations}
\end{table}
We abstract the growing database as a stream of logical updates, denoted by $U = \{u_1, u_2,...\}$, where $u_j\in U$ denotes the logical update at time $j$. $u_j$ can be either a record or empty (denotes no record arrives at time $j$). We define a prefix of stream $U$ at time $t$ as $U_t = \{u_1, u_2, ...,u_t\}$. 
\begin{definition}[Neighboring Stream Prefix] Two stream prefixes $U_t$, and $U'_t$ are considered neighbors if they
differ by the addition or removal of a single tuple, i.e. $|U_t \oplus
 U'_t| = 1$, where $\oplus$ denote symmetric difference. 
\end{definition}

\begin{definition}[$\epsilon$-differential privacy] Let $\mathcal{A}$ be a randomized mechanism that takes as input of a stream prefix. $\mathcal{A}$ satisfies $\epsilon$-differential privacy if for any pair of neighboring prefix $U_t$ and $U'_t$, for all $t$ and $\forall O \subset \mathcal{O}$, where $\mathcal{O}$ denotes all possible outputs,

$$\textup{Pr}[\mathcal{A}(U_t)\in O] \leq e^{\epsilon}\textup{Pr}[\mathcal{A}(U'_t)\in O]$$
\end{definition}


\subsection{Private Join over Dynamic Data}

We begin by introducing some main notations that is used for security model definition. A summary of basic concepts and notations is provided in Table~\ref{tab:notations}.  
\begin{definition}[update pattern]
The update pattern of party $x$ is the function family of $\upatt^{x} = \{\upatt^{x}_t\}_{t\in\mathbb{N}^{+}\land t\in T}$, with:
$$\upatt_{t}^{x}\left(\mathcal{D}_{x}(t)\right) = \left(t, |\mathcal{D}_x(t)|\right)$$
\end{definition}
\begin{definition}[join pattern]
Given two parties $A$, $B$, with corresponding logical growing databases,$\mathcal{D}_A$, and $\mathcal{D}_B$, respectively. Let $T$ as the collection of times when $A$, $B$ recomputes the joint table. Then the joint pattern is defined as the function family of $\jpatt = \{\jpatt_t\}_{t\in\mathbb{N}^{+}\land t\in T}$, with:
$$\jpatt_{t}\left(\mathcal{D}_{A}(t), \mathcal{D}_B(t)\right) = \left(t, |\mathcal{D}_A(t) \bowtie \mathcal{D}_B(t)|\right)$$
\end{definition}


\begin{definition}[DP-Join] A join mechanism $F:\mathcal{D}_A \times \mathcal{D}_B \rightarrow \mathcal{O}$ is said to be $(\epsilon_A, \epsilon_B, \delta_A, \delta_B)$-DP Join, if for any neighboring database pair $(\mathcal{D}_B, \mathcal{D}'_B)$, and any $O \in \mathcal{O}$, it satisfies:
\begin{equation}
    \begin{split}
         \textup{Pr}\left[(F(\mathcal{D}_A, \mathcal{D}_B) \in O\right] \leq e^{\epsilon_B} \textup{Pr}\left[F(\mathcal{D}_A, \mathcal{D}'_B)\in O \right] + \delta_B
    \end{split}
\end{equation}
and the same holds for $F$ over $(\mathcal{D}_A, \mathcal{D}_B)$ and $(\mathcal{D}'_A, \mathcal{D}_B)$ with parameters $\epsilon_A$, and $\delta_A$. If $\epsilon_A = \epsilon_B = \epsilon$ and $\delta_A = \delta_B=\delta$, then we simplify the notation as $(\epsilon,\delta)$-DP Join. 
\end{definition}

\begin{definition}[SIM-CDP-Join]
A 2 party secure join protocol $\Pi$ for computing the join functionality $f:\mathcal{D}_A \times \mathcal{D}_B \rightarrow \mathcal{O}$ is said to be $(\epsilon, \delta)$-SIM-CDP-Join if there exists a p.p.t. simulator $\mathcal{S}$ with only access to the output of a $(\epsilon, \delta)$-DP-Join mechanism $F$, then for any pair of growing database $(\mathcal{D}_A, \mathcal{D}_B)$, and any p.p.t. adversary $\mathcal{A}$. The adversary's advance satisfies:
\begin{equation}
    \begin{split}
        & \textup{Pr}\left[\mathcal{A}\left(\vi^{\Pi}(\mathcal{D}_A, \mathcal{D}_B)=1\right)\right] \\
        & \leq  \textup{Pr}\left[\mathcal{A}\left(\vi^{\mathcal{S}}(F(\mathcal{D}_A, \mathcal{D}_B))\right)=1\right] + \negl(\kappa)
    \end{split}
\end{equation}
where $\vi^{\Pi}$, and $\vi^{\mathcal{S}}$ denotes the adversary's view against the protocol and the simulator's outputs, respectively.
\end{definition}

\begin{figure}
    \centering
    \noindent\fbox{%
    \small
    \parbox{0.4\textwidth}{%
    \begin{center} {\bf Ideal functionality $\mathcal{F}_{\texttt{join}}$ for two-sided output\\}\end{center}\\
    {\bf Parameters}: Two parties $A$ and $B$, each holds an instance of growing database, denoted as $\mathcal{D}_{A}$, and $\mathcal{D}_B$, respectively. A set of time stamps $T=\{t_1, t_2, t_3,...\}$ denotes the collections of times when $A$, $B$ jointly re-computes the join table.\\
 %Receiver's set is of size $N_{Y}$ and sender's set is of size $N_{X}$.\\
    {\bf Functionality}: For each time $t_i\in T$, $A$ inputs $\mathcal{D}_A(t_i)$, and $B$ inputs $\mathcal{D}_B(t_i)$, where $\mathcal{D}_x(t_i) | x \in (A,B)$ denotes the logical database instance for corresponding party at time $t_i$. The functionality outputs $\left(|\mathcal{D}_A(t_i) \bowtie \mathcal{D}_B(t_i)|, |\mathcal{D}_B(t_i)|, |\mathcal{D}_A(t_i)|\right)$.
    }% fbox
}%  } parbox 

\caption{Ideal functionality}
\label{fig:ideal}
\end{figure}


%\textcolor{red}{Q: Privacy composition?}\\
%\textcolor{red}{If new records can join with old records, how privacy is composed?}
%\textcolor{red}{Let $T = \{t_1, t_2, t_3, ..., t_k\}$ denotes a collections of times when join table is recomputed (total $k$ times). Let $\gamma^{A}_1 = \mathcal{D}_{A}(t_1) - \mathcal{D}_{A}(0)$, $\gamma^{A}_2 = \mathcal{D}_{A}(t_2) - \mathcal{D}_{A}(t_1)$, ...}

%Next, we abstract the view of each party over the protocol execution.

An ideal functionality that describes private join computing over dynamic data. Figure~\ref{fig:ideal} shows the ideal functionality. According to this ideal functionality, we abstract the view of each party over an secure join protocol $\Pi$. Party $A$'s view over the protocol can be written as 
\begin{equation}
    \begin{split}
        & \vi^{\Pi}(\mathcal{D}_A, \mathcal{D}_B) = \\ 
        & \left(\upatt^{A}(\mathcal{D}_A), \upatt^{B}(\mathcal{D}_B), \jpatt(\mathcal{D}_A, \mathcal{D}_B) \right)
    \end{split}
\end{equation}


%where $r$ denotes party $A$'s internal randomness. That is say, besides self-randomness, party $A$ can observe party $B$'s update pattern as well as the joint pattern. The party $B$'s view is analogous.

\eat{

We prove security of our proposed protocol in the standard semi-honest simulation-based paradigm. In other word, we say that the
protocol securely realizes the functionality $\mathcal{F}_{\texttt{join}}$, if correct, exists two simulators p.p.t. simulators $\texttt{Sim}_{R}, \texttt{Sim}_S$ with the following properties. The simulator $\texttt{Sim}_{R}$ takes the receiver’s set and the intersection as input, and needs to generate a transcript for the protocol execution that is indistinguishable from the receiver’s view of the real interaction. $\texttt{Sim}_{S}$ is similarly defined, with the exception of not taking the intersection as input.

Joint pattern, formally we define the join pattern as the function family of $\texttt{JoinPatt}(\mathcal{D}_R, \mathcal{D}_S) = \{\texttt{JoinPatt}_t\}_{t\in t' \wedge t \in \mathbb{N}^{+}}$, where $t'$ is the set of times when join happens and $\texttt{JoinPatt}_t = (t, |X_t\cap Y_t|)$. $X_t$ and $Y_t$ corresponds to the inputs of sender and receiver with respect to time $t$.

Receiver's update pattern, the receiver's update pattern is defined as the function family of $\texttt{RecUpdatPatt}(\mathcal{D}_R) = \{\texttt{RecUpdatPatt}_t\}_{t\in t' \wedge t \in \mathbb{N}^{+}}$, where $\texttt{RecUpdatPatt}_t = (t, |Y_t|)$.

Sender's update pattern, the sender's update pattern is defined as the function family of $\texttt{SeUpdatPatt}(\mathcal{D}_S) = \{\texttt{SeUpdatPatt}_t\}_{t\in t' \wedge t \in \mathbb{N}^{+}}$, where $\texttt{SeUpdatPatt}_t = (t, |X_t|)$.

We profile the leakage revealed to the sender the is function over join pattern and the receiver's pattern, written as $\mathcal{L} (\texttt{JoinPatt}, \texttt{RecUpdatPatt})$, and the leakage revealed to the receiver as $\mathcal{L} (\texttt{JoinPatt}, \texttt{SeUpdatPatt})$

Then we should guarantee DP from 2 perspectives:

1. For any neighboring $\mathcal{D}_S, \mathcal{D}'_S$, it satisfies $$\frac{\textup{Pr}\left[ \mathcal{L} (\texttt{JoinPatt}, \texttt{SeUpdatPatt}(\mathcal{D}_S)) \right]}{\textup{Pr}\left[ \mathcal{L} (\texttt{JoinPatt}, \texttt{SeUpdatPatt}(\mathcal{D}'_S)) \right]} \leq e^{\epsilon}$$
}

